A Coding Theorem for Bipartite Unitaries in Distributed Quantum Computation

We analyze implementations of bipartite unitaries by means of local operations and classical communication (LOCC) assisted by shared entanglement. We employ concepts and techniques developed in quantum Shannon theory to study an asymptotic scenario, in which two distant parties perform the same bipartite unitary on infinitely many pairs of inputs. We analyze minimum cost of entanglement and classical communication per copy. For two-round LOCC protocols, we derive a single-letter formula for the minimum cost of entanglement and classical communication, under an additional requirement that the error converges to zero faster than $1/n^4$, where $n$ is the number of input pairs. The formula is given by the "Markovianizing cost" of a tripartite state associated with the unitary, which can be computed by a finite-step algorithm. We also derive a lower bound on the minimum cost of resources, which applies for protocols with arbitrary number of rounds.

==> DQC (IEEE final manuscript)/commands.tex <==
\newcommand{\bra}[1]{\mbox{$\left\langle#1\right|$}}
\newcommand{\ket}[1]{\mbox{$\left|#1\right\rangle$}}
\newcommand{\inpro}[2]{\mbox{$\left\langle#1|#2\right\rangle$}}
\newcommand{\outpro}[2]{\mbox{$\ket{#1}\!\bra{#2}$}}
\newcommand{\proj}[1]{\mbox{$\ket{#1}\!\bra{#1}$}}
\newcommand{\kakko}[1]{\mbox{$\left(#1\right)$}}
\newcommand{\proof}{\noindent{\bf Proof.}  }
\newcommand{\ave}[1]{\mbox{$\left\langle#1\right\rangle$}}
\newcommand{\eq}[1]{Eq.(\ref{eq:#1})}
\newcommand{\sect}[1]{Sec.\,\ref{sec:#1}}
\newcommand{\ep}[1]{\noindent{\underline{\bf EP{#1}:}}}


 

==> DQC (IEEE final manuscript)/preferences_ieee.tex <==

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{thm}{ Theorem}
\newtheorem{dfn}[thm]{ Definition}
\newtheorem{lmm}[thm]{ Lemma}
\newtheorem{exa}[thm]{ Example}
\newtheorem{crl}[thm]{ Corollary}
\newtheorem{cjt}[thm]{ Conjecture}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{prf}{ Proof:}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{skprf}{ Sketch of the proof.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{outprf}{ Outline of the proof.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{prftyp}{ Proof of Theorem \ref{thm:typicalsubspace}.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{prfconv}{ Proof of Theorem \ref{thm:misoptach}.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{rmk}{ Remark.}}

\renewcommand{\theprf}{}
\renewcommand{\theprftyp}{}
\renewcommand{\theoutprf}{}
\renewcommand{\theprfconv}{}
\renewcommand{\thermk}{}



  
